The Influence of Stellar Chromospheres and Coronae on Exoplanet Transmission Spectroscopy

A main source of bias in transmission spectroscopy of exoplanet atmospheres is magnetic activity of the host star in the form of stellar spots, faculae or flares. However, the fact that main-sequence stars have a chromosphere and a corona, and that these optically thin layers are dominated by line emission may alter the global interpretation of the planetary spectrum, has largely been neglected. Using a JWST NIRISS/SOSS data set of hot Jupiter HAT-P-18 b, we show that even at near-IR and IR wavelengths, the presence of these layers leads to significant changes in the transmission spectrum of the planetary atmosphere. Accounting for these stellar outer layers thus improves the atmospheric fit of HAT-P-18 b, and increases its best-fit atmospheric temperature from 536 K to 736 K, a value much closer to the predicted equilibrium temperature of 852 K. Our analysis also decreases the best-fit abundance of CO2 by almost an order of magnitude. The approach provides a new window to the properties of chromospheres/corona in stars other than our Sun.

==> journal_abbrev.tex <==
% \newcommand\mnras{MNRAS}
% \newcommand\nat{Nature}
% \newcommand\procspie{Proc. SPIE}
% \newcommand\pasp{PASP}
% \newcommand\aap{A\&A}
% \newcommand\icarus{Icarus}
% \newcommand\apj{The Astrophysical Journal}
% \newcommand\apjl{The Astrophysical Journal, Letters}
% \newcommand\apjs{The Astrophysical Journal, Supplement}
% \newcommand\aj{The Astronomical Journal}
% \newcommand\solphys{Sol. Phys.}
% \newcommand\pasj{Publications of the ASJ}
% \newcommand\aaps{Astronomy and Astrophysics, Supplement}
% \newcommand\memsai{Mem. Societa Astronomica Italiana}
% \newcommand\ssr{Space Science Reviews}
% \newcommand\araa{Ann .Rev. Astron. Astrophys.}

% from https://communities.springernature.com/posts/latex-tips-for-nature-astronomy-submissions
\newcommand{\actaa}{Acta Astron.}   % Acta Astronomica
\newcommand{\araa}{Annu. Rev. Astron. Astrophys.}   % Annual Review of Astron and Astrophys
\newcommand{\areps}{Annu. Rev. Earth Planet. Sci.} % Annual Review of Earth and Planetary Science
\newcommand{\aar}{Astron. Astrophys. Rev.} % Astrononmy and Astrophysics Review
\newcommand{\ab}{Astrobiology}    % Astrobiology
\newcommand{\aj}{Astron. J.}   % Astronomical Journal
\newcommand{\ac}{Astron. Comput.} % Astronomy and Computing
\newcommand{\apart}{Astropart. Phys.} % Astroparticle Physics
\newcommand{\apj}{Astrophys. J.}   % Astrophysical Journal
\newcommand{\apjl}{Astrophys. J. Lett.}   % Astrophysical Journal, Letters
\newcommand{\apjs}{Astrophys. J. Suppl. Ser.}   % Astrophysical Journal, Supplement
\newcommand{\ao}{Appl. Opt.}   % Applied Optics
\newcommand{\apss}{Astrophys. Space Sci.}   % Astrophysics and Space Science
\newcommand{\aap}{Astron. Astrophys.}   % Astronomy and Astrophysics
\newcommand{\aapr}{Astron. Astrophys. Rev.}   % Astronomy and Astrophysics Reviews
\newcommand{\aaps}{Astron. Astrophys. Suppl.}   % Astronomy and Astrophysics, Supplement
\newcommand{\baas}{Bull. Am. Astron. Soc.}   % Bulletin of the AAS
\newcommand{\caa}{Chin. Astron. Astrophys.}   % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{Chin. J. Astron. Astrophys.}   % Chinese Journal of Astronomy and Astrophysics (now RAA)
\newcommand{\cqg}{Class. Quantum Gravity}    % Classical and Quantum Gravity
\newcommand{\epsl}{Earth Planet. Sci. Lett.}    % Earth and Planetary Science Letters
\newcommand{\frass}{Front. Astron. Space Sci.}    % Frontiers in Astronomy and Space Sciences
\newcommand{\gal}{Galaxies}    % Galaxies
\newcommand{\gca}{Geochim. Cosmochim. Acta}   % Geochimica Cosmochimica Acta
\newcommand{\grl}{Geophys. Res. Lett.}   % Geophysics Research Letters
\newcommand{\icarus}{Icarus}   % Icarus
\newcommand{\ija}{Int. J. Astrobiol.} % International Journal of Astrobiology
\newcommand{\jatis}{J. Astron. Telesc. Instrum. Syst.}  % Journal of Astronomical Telescopes, Instruments, and Systems 
\newcommand{\jcap}{J. Cosmol. Astropart. Phys.}   % Journal of Cosmology and Astroparticle Physics
\newcommand{\jgr}{J. Geophys. Res.}   % Journal of Geophysics Research
\newcommand{\jgrp}{J. Geophys. Res.: Planets}    % Journal of Geophysics Research: Planets
\newcommand{\jqsrt}{J. Quant. Spectrosc. Radiat. Transf.} % Journal of Quantitiative Spectroscopy and Radiative Transfer
\newcommand{\lrca}{Living Rev. Comput. Astrophys.}    % Living Reviews in Computational Astrophysics
\newcommand{\lrr}{Living Rev. Relativ.}    % Living Reviews in Relativity
\newcommand{\lrsp}{Living Rev. Sol. Phys.}    % Living Reviews in Solar Physics
\newcommand{\memsai}{Mem. Soc. Astron. Italiana}   % Mem. Societa Astronomica Italiana
\newcommand{\maps}{Meteorit. Planet. Sci.} % Meteoritics and Planetary Science
\newcommand{\mnras}{Mon. Not. R. Astron. Soc.}   % Monthly Notices of the RAS
\newcommand{\nat}{Nature} % Nature
\newcommand{\nastro}{Nat. Astron.} % Nature Astronomy
\newcommand{\ncomms}{Nat. Commun.} % Nature Communications
\newcommand{\ngeo}{Nat. Geosci.} % Nature Geoscience
\newcommand{\nphys}{Nat. Phys.} % Nature Physics
\newcommand{\na}{New Astron.}   % New Astronomy
\newcommand{\nar}{New Astron. Rev.}   % New Astronomy Review
\newcommand{\physrep}{Phys. Rep.}   % Physics Reports
\newcommand{\pra}{Phys. Rev. A}   % Physical Review A: General Physics
\newcommand{\prb}{Phys. Rev. B}   % Physical Review B: Solid State
\newcommand{\prc}{Phys. Rev. C}   % Physical Review C
\newcommand{\prd}{Phys. Rev. D}   % Physical Review D
\newcommand{\pre}{Phys. Rev. E}   % Physical Review E
\newcommand{\prl}{Phys. Rev. Lett.}   % Physical Review Letters
\newcommand{\psj}{Planet. Sci. J.}   % Planetary Science Journal
\newcommand{\planss}{Planet. Space Sci.}   % Planetary Space Science
\newcommand{\pnas}{Proc. Natl Acad. Sci. USA}   % Proceedings of the US National Academy of Sciences
\newcommand{\procspie}{Proc. SPIE}   % Proceedings of the SPIE
\newcommand{\pasa}{Publ. Astron. Soc. Aust.}   % Publications of the Astron. Soc. of Australia
\newcommand{\pasj}{Publ. Astron. Soc. Jpn}   % Publications of the Astron. Soc. of Japan (note no full stop following Jpn)
\newcommand{\pasp}{Publ. Astron. Soc. Pac.}   % Publications of the Astron. Soc. of the Pacific
\newcommand{\raa}{Res. Astron. Astrophys.} % Research in Astronomy and Astrophysics (formerly CJAA)
\newcommand{\rmxaa}{Rev. Mexicana Astron. Astrofis.}   % Revista Mexicana de Astronomia y Astrofisica
\newcommand{\sci}{Science} % Science
\newcommand{\sciadv}{Sci. Adv.} % Science Advances
\newcommand{\solphys}{Sol. Phys.}   % Solar Physics
\newcommand{\sovast}{Soviet Astron.}   % Soviet Astronomy
\newcommand{\ssr}{Space Sci. Rev.}   % Space Science Reviews
\newcommand{\uni}{Universe} % Universe
